Vision-Language Generative Model for View-Specific Chest X-ray Generation

Synthetic medical data generation has opened up new possibilities in the healthcare domain, offering a powerful tool for simulating clinical scenarios, enhancing diagnostic and treatment quality, gaining granular medical knowledge, and accelerating the development of unbiased algorithms. In this context, we present a novel approach called ViewXGen, designed to overcome the limitations of existing methods that rely on general domain pipelines using only radiology reports to generate frontal-view chest X-rays. Our approach takes into consideration the diverse view positions found in the dataset, enabling the generation of chest X-rays with specific views, which marks a significant advancement in the field. To achieve this, we introduce a set of specially designed tokens for each view position, tailoring the generation process to the user's preferences. Furthermore, we leverage multi-view chest X-rays as input, incorporating valuable information from different views within the same study. This integration rectifies potential errors and contributes to faithfully capturing abnormal findings in chest X-ray generation. To validate the effectiveness of our approach, we conducted statistical analyses, evaluating its performance in a clinical efficacy metric on the MIMIC-CXR dataset. Also, human evaluation demonstrates the remarkable capabilities of ViewXGen, particularly in producing realistic view-specific X-rays that closely resemble the original images.

==> source/11.apd_single.tex <==
\subsection{Chest X-ray Generation}
We study the advantage of training a unified model for multi-view chest X-ray generation.

We compare our model with Single$_{AP}$, Single$_{PA}$, and Single$_{LAT.}$.
Table~\ref{tab:cxr_fid_classification_single} shows the results.
In terms of the statistical metric (FID, the lower the better), \model outperforms the single models only in the PA case.
In terms of the clinical efficacy metric (14-diagnosis classification), however, it shows significantly superior performance than all single models: AUROC (\model – Single$_{AP}$ = 0.066, [95\% CI 0.065, 0.066], \model – Single$_{PA}$ = 0.007, [95\% CI 0.007, 0.008], and \model – Single$_{LAT.}$ = 0.027, [95\% CI 0.027, 0.028]).
This suggests that training a model to generate multiple views helps the model to correctly capture the abnormalities described in the report.

From these results, we demonstrate that \model is comparable, if not superior, to the various single models tailored to generate only its specific modality.
Specifically, only the mean FID difference of PA outperforms the single model in the statistical metric, but except for this, \model significantly outperforms the single models across all metrics.
This suggests that our model can generate multi-view chest X-rays with clinically meaningful information.
We can conclude that bidirectional training has a synergistic effect on generation tasks and also can save time and computational costs, as opposed to training multiple single models.

\input{tables/tab1_cxr_fid_classification_single}

\subsection{Radiology Report Generation}
As shown in Table~\ref{tab:report_bleu_labeler_single}, we compare our model with Single$_{report}$.
We can observe that \model significantly outperforms Single$_{report}$ in both statistical and clinical efficacy metrics (mean CheXpert F1 difference = 0.067, [95\% CI 0.066, 0.067]). This indicates that combining chest X-ray image generation as a target can effectively capture local regions that encourage the model to generate more precise reports containing abnormal findings.
\input{tables/tab2_report_bleu_labeler_single}
